Graphical Gaussian Process Regression Model for Aqueous Solvation Free Energy Prediction of Organic Molecules in Redox Flow Battery

The solvation free energy of organic molecules is a critical parameter in determining emergent properties such as solubility, liquid-phase equilibrium constants, and pKa and redox potentials in an organic redox flow battery. In this work, we present a machine learning (ML) model that can learn and predict the aqueous solvation free energy of an organic molecule using Gaussian process regression method based on a new molecular graph kernel. To investigate the performance of the ML model on electrostatic interaction, the nonpolar interaction contribution of solvent and the conformational entropy of solute in solvation free energy, three data sets with implicit or explicit water solvent models, and contribution of conformational entropy of solute are tested. We demonstrate that our ML model can predict the solvation free energy of molecules at chemical accuracy with a mean absolute error of less than 1 kcal/mol for subsets of the QM9 dataset and the Freesolv database. To solve the general data scarcity problem for a graph-based ML model, we propose a dimension reduction algorithm based on the distance between molecular graphs, which can be used to examine the diversity of the molecular data set. It provides a promising way to build a minimum training set to improve prediction for certain test sets where the space of molecular structures is predetermined.

==> concl.tex <==



==> support.tex <==
\section{Support Material}

\subsection{Details of GPR}
In the GPR method, the mean and covariance functions $\mu(\bm x)$ and 
$k(\bm x,\bm x')$ are obtained by identifying their hyperparameters via 
maximizing the log marginal likelihood~\cite{williams2006gaussian}:
%-------------------------------------------------------------------------------
\begin{equation}
  \label{eq:lml}
  \ln L=-\dfrac{1}{2}(\bm y-\bm\mu)^\trans \tensor C^{-1} (\bm
  y-\bm\mu)-\dfrac{1}{2}\ln |\tensor C|-\dfrac{N}{2}\ln 2\pi.
\end{equation}
%-------------------------------------------------------------------------------

Moreover, to account for the observation noise, one can assume that the noise is
independent and identically distributed (i.i.d.) Gaussian random variables with
zero mean and variance $\delta^2$, and replace $\tensor C$ with 
$\tensor C+\delta^2\tensor I$. In this study, we assume that observations 
$\bm y$ are noiseless. If $\tensor C$ is not invertible or its condition number
is very large, one can add a small regularization term $\alpha\tensor I$
($\alpha$ is a small positive real number) to $\tensor C$, % such that it becomes full rank. 
which is equivalent to assuming there
is an observation noise. In addition, $\hat s$ can be used in global
optimization, or in the greedy algorithm to identify locations of additional
observations. 

Given a stationary covariance function, the covariance matrix $\tensor C$ can be written as
$\tensor C=\sigma^2\tensor \Psi$, where
$\Psi_{ij}=\exp(-\frac{1}{2}\Vert\bm x^{(i)}-\bm x^{(j)}\Vert_w^2)$. The estimators of $\mu$ and $\sigma^2$, denoted as $\hat\mu$ and
$\hat\sigma^2$, are
%-------------------------------------------------------------------------------
\begin{equation}
\label{eq:krig_est}
   \hat\mu=\dfrac{\bm 1^\trans \tensor\Psi^{-1}\bm y}
                  {\bm 1^\trans\tensor\Psi^{-1}\bm 1}, \qquad
   \hat\sigma^2=\dfrac{(\bm y-\bm 1\hat\mu)^\trans\tensor\Psi^{-1}(\bm y-\bm 1\hat\mu)}{N},
\end{equation}
%-------------------------------------------------------------------------------
where $\bm 1$ is a constant vector consisting of $1$s~\cite{forrester2008engineering}. 
It is also common to set $\mu=0$~\cite{williams2006gaussian}. The hyperparameters $\sigma$ and $l_i$ are 
identified by maximizing the log marginal likelihood in Eq.~\eqref{eq:lml}. The terms
$\hat y(\bm x^*)$ and $\hat s^2(\bm x^*)$ in Eq.~\eqref{eq:krig} take the 
following form:
%-------------------------------------------------------------------------------
\begin{align}
\label{eq:krig_mean}
\hat y(\bm x^*) & = \hat\mu + \bm\psi^\trans\tensor\Psi^{-1}(\bm y-\bm 1\hat\mu), \\
\label{eq:krig_var}
\hat s^2(\bm x^*) & = \hat\sigma^2\left(1-\bm\psi^\trans\tensor\Psi^{-1}\bm\psi\right),
\end{align}
%-------------------------------------------------------------------------------
where $\bm\psi=\bm\psi(\bm x^*)$ is a (column) vector consisting of correlations between the observed data and the
prediction, i.e., $\psi_i=\frac{1}{\sigma^2}k(\bm x^{(i)},\bm x^*)$.
%-------------------------------------------------------------------------------


\subsection{Details of GPR using graph kernel}

In Eq.~\eqref{eq:distance}, the straightforward enumeration is impossible, because $\ell$ spans from $1$ to $\infty$. Nevertheless, Eq.~\eqref{eq:distance} can be reformulated under the spirit of dynamic programming as follows:
\begin{equation}
    K(G, G')=\sum_{h_1\in V, h'_1\in V'}p_s(h_1)p_s'(h'_1)K_v(h_1, h_1')R_{\infty}(h_1,h_1'),
\end{equation}
where $R_{\infty}$ is the solution to the following (linear) equilibrium equation
\begin{equation}
 R_{\infty}(h_1,h_1')=p_q(h_1)p'_q(h_1')+\sum_{i\in V, j\in V'}t(i,j,h_1,h_1')R_{\infty}(i,j), \label{eq:rinf}
\end{equation}
where 
\begin{equation}
    t(i,j,h_1,h_1')\defeq p_t(i|h_1) p_t'(j|h_1')K_v(v_i,v_j)K_e(e_{ih_1},e_{jh_1'}).
\end{equation}

Equation \ref{eq:rinf} exhibits a Kronecker product structure, which can be readily recognized in matrix form~\cite{tang2019prediction}:
\begin{equation}
  \mathbf{r}_\infty = \mathbf{q} \otimes \mathbf{q}' + \left[ \left( \mathbf{P} \otimes \mathbf{P}' \vphantom{\overset{\kappa_\mathrm{v}}{\smallotimes}} \right) \odot \left( \mathbf{E} \overset{\kappa_\mathrm{e}}{\smallotimes} \mathbf{E}' \right) \right] \cdot \mathbf{diag}\left( \mathbf{v} \overset{\kappa_\mathrm{v}}{\smallotimes} \mathbf{v}' \right) \cdot \mathbf{r}_\infty, \label{eq:r-infinity-linear-system}
\end{equation}
where
\begin{itemize}[label=,leftmargin=8em]
  \item[$\mathbf{v}\phantom{'}$] is the vertex label vector of $G$ with $\mathbf{v}_i = v_i$;
  \item[$\mathbf{p}\phantom{'}$] is the starting probability vector of $G$ with $\mathbf{p}_i = p_s(v_i)$;
  \item[$\mathbf{q}\phantom{'}$] is the stopping probability vector of $G$ with $\mathbf{q}_i = p_q(v_i)$;
  \item[$\mathbf{P}\phantom{'}$] is the transition probability matrix of $G$ defined as $\mathbf{D}^{-1} \mathbf{A}$;
  \item[$\mathbf{E}\phantom{'}$] is the edge label matrix of $G$ with $\mathbf{E}_{ij} = e_{ij}$;
  \item[$\mathbf{v}'$, $\mathbf{p}'$, $\mathbf{q}'$, $\mathbf{P}'$, $\mathbf{E}'$] are the corresponding vectors and matrices for $G'$;
  \item[$\overset{\kappa_\mathrm{v}}{\smallotimes}\phantom{'}$] is the generalized Kronecker product between $\mathbf{v}$ and $\mathbf{v}'$ with respect to microkernel $\kappa_\mathrm{v}$;
  \item[$\overset{\kappa_\mathrm{e}}{\smallotimes}\phantom{'}$] is the generalized Kronecker product between $\mathbf{E}$ and $\mathbf{E}'$ with respect to microkernel $\kappa_\mathrm{e}$.
\end{itemize}

